General Purpose Verification for Chain of Thought Prompting

Many of the recent capabilities demonstrated by Large Language Models (LLMs) arise primarily from their ability to exploit contextual information. In this paper, we explore ways to improve reasoning capabilities of LLMs through (1) exploration of different chains of thought and (2) validation of the individual steps of the reasoning process. We propose three general principles that a model should adhere to while reasoning: (i) Relevance, (ii) Mathematical Accuracy, and (iii) Logical Consistency. We apply these constraints to the reasoning steps generated by the LLM to improve the accuracy of the final generation. The constraints are applied in the form of verifiers: the model itself is asked to verify if the generated steps satisfy each constraint. To further steer the generations towards high-quality solutions, we use the perplexity of the reasoning steps as an additional verifier. We evaluate our method on 4 distinct types of reasoning tasks, spanning a total of 9 different datasets. Experiments show that our method is always better than vanilla generation, and, in 6 out of the 9 datasets, it is better than best-of N sampling which samples N reasoning chains and picks the lowest perplexity generation.

==> tables/unfaithful_cot_reasoning_example.tex <==
\begin{tabular}{ll}
    \toprule
    \textbf{\footnotesize{Problem}} & \begin{tabular}[c]{@{}l@{}}A concert ticket costs \$40.\\Mr. Doe buys 10 tickets. \\Mr. Benson buys 12. \\For every ticket bought after 10, Mr. Benson \\receives a 5\% discount. \\How much did Mr. Benson pay in all? \end{tabular}\\
    \addlinespace[0.25em]
    \midrule
    \addlinespace[0.25em]
    \textbf{\footnotesize{
     \begin{tabular}[c]{@{}l@{}}Step by Step\\Solution\end{tabular}
    }} & \begin{tabular}[c]{@{}l@{}}
    1. Mr. Doe paid in total 10 * \$40 = \$400. (\textcolor{red}{Irrelevant})\\
    2. Without the discount, Mr. Benson paid in total \\12 * \$40 = \$480.\\
    3. Mr. Benson received a discount of \\2 * (\$40 - \$38) = \$4  (\$2 per ticket)\\
    4. So Mr. Benson received a discount of \$0.02 \\per ticket. (\textcolor{red}{Inconsistent})\\
    5. With discount, Mr. Benson paid \$480 - 2 * \$2 = \$478.\\
    Therefore, Mr. Benson paid \$476. (\textcolor{red}{Incorrect calculations})\\
    \end{tabular} \\
    \bottomrule
\end{tabular}
